Active T1 transitions in cellular networks

In amorphous solids as in tissues, neighbor exchanges can relax local stresses and allow the material to flow. In this paper, we use an anisotropic vertex model to study T1 rearrangements in polygonal cellular networks. We consider two different physical realizations of the active anisotropic stresses: (i) anisotropic bond tension and (ii) anisotropic cell stress. Interestingly, the two types of active stress lead to patterns of relative orientation of T1 transitions and cell elongation that are different. Our work suggests that these two realizations of anisotropic active stresses can be observed \textit{in vivo}. We describe and explain these results through the lens of a continuum description of the tissue as an anisotropic active material. We furthermore discuss the energetics of the dynamic tissue and express the energy balance in terms of internal elastic energy, mechanical work, chemical work and heat. This allows us to define active T1 transitions that can perform mechanical work while consuming chemical energy.

==> my_macros.tex <==
%%%%% packages added by Charlie
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bbold} %% for \mathbb etc
\usepackage{color}
\usepackage[dvipsnames]{xcolor}

%%%%%%%%
\usepackage[utf8]{inputenc}
\usepackage{subfigure}
\usepackage{xifthen}
\usepackage{graphicx}
\usepackage{hyphenat}
\usepackage{hhline}
\usepackage{upgreek}
\usepackage{bm}
\usepackage{xcolor}

\usepackage{subfiles} % Best loaded last in the preamble

%%%%%%%%%%%%%%%%%%%%%%
%% ### References.  %%
%%%%%%%%%%%%%%%%%%%%%%%

% for greater/lower or similar
\def\simge{\mathrel{%
   \rlap{\raise 0.511ex \hbox{$>$}}{\lower 0.511ex \hbox{$\sim$}}}}
\def\simle{\mathrel{
   \rlap{\raise 0.511ex \hbox{$<$}}{\lower 0.511ex \hbox{$\sim$}}}}

\newcommand{\aref}[1]{App.~\ref{app:#1}}
\newcommand{\arefs}[1]{Apps.~\ref{app:#1}}
\newcommand{\alabel}[1]{\label{app:#1}}

\newcommand{\tref}[1]{Table~\ref{table:#1}}
\newcommand{\trefs}[1]{Tables~\ref{table:#1}}
\newcommand{\tlabel}[1]{\label{table:#1}}

\newcommand{\fref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\fsref}[1]{Fig. S\ref{fig:#1}}
\newcommand{\frefs}[1]{Figs.~\ref{fig:#1}}
\newcommand{\flabel}[1]{\label{fig:#1}}

\newcommand{\eref}[1]{Eq.~\ref{eqn:#1}}
\newcommand{\erefs}[1]{Eqs.~\ref{eqn:#1}}
\newcommand{\erefstwo}[2]{Eqs.~\ref{eqn:#1}~and~\ref{eqn:#2}}
\newcommand{\erefsrange}[2]{Eqs.~\ref{eqn:#1}-\ref{eqn:#2}}
\newcommand{\elabel}[1]{\label{eqn:#1}}

\newcommand{\chref}[1]{chapter~\ref{ch:#1}}
\newcommand{\chrefs}[1]{chapters~\ref{ch:#1}}
\newcommand{\chlabel}[1]{\label{ch:#1}}

\newcommand{\secref}[1]{section~\ref{sec:#1}}
\newcommand{\secrefs}[1]{sections~\ref{sec:#1}}
\newcommand{\seclabel}[1]{\label{sec:#1}}

\newcommand{\ssref}[1]{section~\ref{ssec:#1}}
\newcommand{\ssrefs}[1]{sections~\ref{ssec:#1}}
\newcommand{\sslabel}[1]{\label{ssec:#1}}


% ### General vector notations
% Bold symbol for vector
\newcommand{\myvec}[1]{\ensuremath{\bm{#1}}}
% Bold symbol with hat for unit vector.
\newcommand{\myunitvec}[1]{\ensuremath{\bm{\hat{#1}}}}
% Math symbol with roman labeled sub and super scripts.
\newcommand{\rmlabel}[3]{\ensuremath{#1_\mathrm{#2}^\mathrm{#3}}}
%General definition for components  of a traceless symmetric tensor T.
\newcommand{\nematicT}[2]{%
\ifthenelse{\isempty{#2}}{\ensuremath{\tilde{#1}_{ij}}}{\ensuremath{\tilde{#1}_{#2}}}%
}
%General definition for components of a tensor T.
\newcommand{\normalT}[2]{%
\ifthenelse{\isempty{#2}}{\ensuremath{#1_{ij}}}{\ensuremath{#1_{#2}}}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% ### Symbols for hydrodynamic models %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Moduli
\newcommand{\shearmod}[0]{\ensuremath{\rmlabel{\mu}{s}{}}}
\newcommand{\bulkmod}[0]{\ensuremath{\rmlabel{\mu}{b}{}}}

% Total shear rate.
\newcommand{\shearv}[1]{%
\ifthenelse{\isempty{#1}}{\nematicT{v}{}}{\nematicT{v}{#1}}%
}
\newcommand{\strainv}[1]{%
\ifthenelse{\isempty{#1}}{\normalT{v}{}}{\normalT{v}{#1}}%
}
\newcommand{\shearrate}[0]{v_0}

% Anisotropic stress.
\newcommand{\shears}[1]{%
\ifthenelse{\isempty{#1}}{\nematicT{\sigma}{}}{\nematicT{\sigma}{#1}}%
}
% Steady state anisotropic stress.
\newcommand{\shearsss}[1]{%
\ifthenelse{\isempty{#1}}{\nematicT{\sigma}{}^\mathrm{ss}}{\nematicT{\sigma}{#1}^\mathrm{ss}}%
}
% Mean cell elongation in hydr.
\newcommand{\shearq}[1]{%
\ifthenelse{\isempty{#1}}{\normalT{q}{}}{\normalT{q}{#1}}%
}
% Cell polarity.
\newcommand{\shearp}[1]{%
\ifthenelse{\isempty{#1}}{\normalT{p}{}}{\normalT{p}{#1}}%
}
% Corotational derivative, continuum theory.
\newcommand{\shearDqDt}[1]{%
\ifthenelse{\isempty{#1}}{\ensuremath{\frac{D\widetilde{q}_{ij}}{Dt}}}{\ensuremath{\frac{D\widetilde{q}_{#1}}{Dt}}}%
}
% Topological rearrangements rate
\newcommand{\shearr}[1]{%
\ifthenelse{\isempty{#1}}{\normalT{r}{}}{\normalT{r}{#1}}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% ### Symbols for vertex models %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Tissue anisotropic active stress.
\newcommand{\shearSact}[1]{%
\ifthenelse{\isempty{#1}}{\normalT{\tilde\Sigma^{\mathrm{a}}}{}}{\normalT{\tilde\Sigma^{\mathrm{a}}}{#1}}%
}
% Tissue anisotropic stress.
\newcommand{\shearS}[1]{%
\ifthenelse{\isempty{#1}}{\nematicT{\Sigma}{}}{\nematicT{\Sigma}{#1}}%
}
% Steady state anisotropic stress.
\newcommand{\shearSss}[1]{%
\ifthenelse{\isempty{#1}}{\nematicT{\Sigma}{}^\mathrm{ss}}{\nematicT{\Sigma}{#1}^\mathrm{ss}}%
}
% Cell elongation for Vertex Model.
\newcommand{\shearQVM}[1]{%
\ifthenelse{\isempty{#1}}{\ensuremath{\normalT{G}{}}}{\ensuremath{\normalT{\widetilde{Q}}{#1}}}%
}
% Mean cell elongation in VM.
\newcommand{\shearQ}[1]{%
\ifthenelse{\isempty{#1}}{\normalT{\widetilde{Q}}{}}{\normalT{\widetilde{Q}}{#1}}%
}
%Steady state cell elongation.
\newcommand{\shearQss}[1]{%
\ifthenelse{\isempty{#1}}{\ensuremath{\normalT{\widetilde{Q}}{}^{\mathrm{ss}}}}{\ensuremath{\normalT{\widetilde{Q}}{#1}^{\mathrm{ss}}}}%
}
%Steady state cell elongation.
\newcommand{\shearqss}[1]{%
\ifthenelse{\isempty{#1}}{\ensuremath{\normalT{q}{}^{\mathrm{ss}}}}{\ensuremath{\normalT{q}{#1}^{\mathrm{ss}}}}%
}
%Topological changes rate.
\newcommand{\shearR}[1]{%
\ifthenelse{\isempty{#1}}{\normalT{R}{}}{\normalT{R}{#1}}%
}
%Corotational derivative.
\newcommand{\shearDQDt}[1]{%
\ifthenelse{\isempty{#1}}{\ensuremath{\frac{D\widetilde{Q}_{ij}}{Dt}}}{\ensuremath{\frac{D\widetilde{Q}_{#1}}{Dt}}}%
}

%Bold face cell polarity and cell elongation tensors.
\newcommand{\vecp}{\widetilde{\bm{p}}}
\newcommand{\vecQ}{\widetilde{\bm{Q}}}



\definecolor{nblue}{RGB}{28,130,185}
\newcommand{\cha}[1]{\textcolor{nblue}{#1}}
\usepackage{amsmath}


%Corotational derivative.
\newcommand{\DDt}[1]{%
\frac{{\rm D}#1}{{\rm D}t}%
}
%inline version
\newcommand{\DDtinline}[1]{%
{\rm D}#1/{\rm D}t%
}

%time derivative.
\newcommand{\ddt}[1]{%
\frac{{\rm d}#1}{{\rm d}t}%
}
%inline version
\newcommand{\ddtinline}[1]{%
{\rm d}#1/{\rm d}t%
}
